Distinguishing Standard Model Extensions using Monotop Chirality at the LHC

We present two minimal extensions of the standard model, each giving rise to baryogenesis. They include heavy color-triplet scalars interacting with a light Majorana fermion that can be the dark matter (DM) candidate. The electroweak charges of the new scalars govern their couplings to quarks of different chirality, which leads to different collider signals. These models predict monotop events at the LHC and the energy spectrum of decay products of highly polarized top quarks can be used to establish the chiral nature of the interactions involving the heavy scalars and the DM. Detailed simulation of signal and standard model background events is performed, showing that top quark chirality can be distinguished in hadronic and leptonic decays of the top quarks.

==> report.tex <==
Dear Editor,

Thank you very much for the report. We enclose below our response to the referee's comments and the modifications we have made to the draft. We are also resubmitting our modified draft. We hope that the new version is ready to be accepted in JHEP.

Sincerely,

Yu Gao
On behalf of authors

----------------------------------------------------------------------------------------------------------------------

1. We tried to differentiate the left-handed and right-handed monotop scenarios in the paper. The models 1 and 2 are two new models with right and left-handed monotop final states respectively. The SM also produces the left handed monotop final states.  The model we use to generate the events for analysis is  model 1 for right-handed top+missing energy final state. In order to generate events for left handed case we modify the model I to couple X to left handed quark and missing energy final state. We use same cross-section and then compare LH and RH scenarios. Now, model 2 can have a different production process which means different couplings and masses of new particles to produce the single top plus missing energy final state. However, the difference in the production process does not change the analysis since our analysis applies cuts on total missing energy, attempts to reconstruct the  top quark and investigate b jet energy distribution. All these selection cuts we have developed can be applied to any scenario of top plus missing energy final state independent of the production process.  

We now have added a couple of lines on page 3 of the modified draft: ``Model 2 can have a different production process compared to the toy model with left-handed top plus missing energy final states which means that the coupling strengths of  the new particles with top quarks are different compared to the toy model. However, the difference in the production process does not change the analysis since our analysis applies cuts on total missing energy, attempts to reconstruct the  top quark and investigate b jet energy distribution. All the selection cuts we have developed can be applied to any scenario of top plus missing energy final state independent of the production process. ''

2. We have used $\lambda=10^{-2}$ and $m_X$=1 TeV to satisfy the current CMS bound as mentioned on page 3. In model 2, if we want to produce the same cross-section in order to satisfy the CMS bound, we need $y$=0.1. We have added a line on page: ''In model 2, if we want to produce less than 20fb cross-section in order to satisfy the CMS bound, we only need $y$<0.8 for 1 TeV scalar.''

